Inherent Failure Modes of Physics-Informed Neural Networks for Buoyancy-Driven Flow: Role of Non-Dimensionalization in Network Training

We investigate the influence of non-dimensionalization on the trainability and accuracy of physics-informed neural networks (PINNs) for buoyancy-driven flows. Using a differentially heated square cavity at $\mathrm{Pr}=0.71$ and $\mathrm{Ra}=10^3$--$10^5$, we compare thermal-diffusive and free-fall velocity scalings under identical training conditions. The free-fall scaling, with a unit buoyancy coefficient, achieves errors below 1.1\% in the mean Nusselt number for $\mathrm{Ra}\le10^4$, whereas the diffusive scaling, with a buoyancy coefficient of $\mathrm{Ra}\,\mathrm{Pr}$, produces errors of 157--650\% and diverges at $\mathrm{Ra}=10^5$. We identify a coefficient-induced gradient imbalance, with the dominant buoyancy-related contribution to the loss gradient scaling as $(\mathrm{Ra}\,\mathrm{Pr})^2$, and confirm it through direct gradient measurements. Neither sparse-data supervision nor adaptive loss weighting resolves the training difficulties under the tested conditions. For unsteady convection, the free-fall PINN accurately predicts long-time heat transfer but fails to capture the transient Nusselt-number overshoot. These findings establish non-dimensionalization as an important design consideration for improving PINN trainability in buoyancy-driven flows.

==> intro.tex <==

\subsection{Physics-informed neural networks}
Physics-informed neural networks (PINNs) approximate the solution of a partial differential equation (PDE) with a neural network trained to minimize the residual of the governing equations at a set of collocation points, together with the boundary and initial conditions, rather than by discretizing the domain onto a mesh. The idea traces back to Lagaris et al.\ \citep{lagaris1998}, who used a neural network trial function constructed to satisfy simple boundary conditions exactly and trained it to satisfy the interior ODE/PDE by minimizing its residual, and was substantially generalized and popularized by Raissi et al.\ \citep{raissi2019}, who combined automatic differentiation with a purely soft (loss-based) treatment of boundary and initial conditions, enabling application to nonlinear PDEs of essentially arbitrary form without deriving problem-specific discretizations. Because the same collocation-and-autodiff machinery applies whether the residual is evaluated at the same points used to fit sparse or noisy observational data, PINNs have proven attractive for inverse and data-assimilation problems, and the framework has since been packaged into general-purpose software such as DeepXDE \citep{lu2021deepxde} and applied across fluid mechanics, heat transfer, solid mechanics, and beyond \citep{karniadakis2021}.

\subsection{Training pathologies and mitigation strategies}
\label{sec:pathologies}
Despite this generality, PINNs are well known to be substantially harder to train to high accuracy than the smooth, convex picture of ``minimize a residual'' suggests. A PINN's loss function sums multiple terms -- typically one or more PDE-residual terms plus boundary- and initial-condition terms -- that are not commensurate in scale, and Wang et al.\ \citep{wang2021} showed, using a neural tangent kernel analysis, that when one term's gradient dominates the others during backpropagation, Adam-based training stalls on the dominated terms regardless of how long training continues; they proposed a learning-rate annealing scheme that reweights loss terms using their relative gradient statistics. McClenny and Braga-Neto \citep{mcclenny2023} took this further with per-collocation-point trainable weights that let the network adaptively concentrate attention on the hardest-to-fit regions of the domain during training. A complementary strategy avoids the imbalance altogether for the terms it can reach: rather than penalizing a boundary-condition mismatch in the loss, Dirichlet (and some Neumann) conditions can be built into the network's output algebraically, via a trial-function ansatz \citep{lagaris1998} or, more generally, via an approximate distance function to the domain boundary \citep{sukumar2022}, removing that term from the loss and its associated gradient competition entirely. All of this work, however, targets imbalance \emph{between} loss terms at a fixed, already-chosen non-dimensionalization of the PDE. The imbalance we study in this paper arises one level earlier -- from the coefficients of the PDE itself, before any such inter-term weighting or hard-constraint scheme is applied -- and, to our knowledge, has not been isolated and quantified as a distinct failure mode in this literature.

\subsection{PINNs for buoyancy-driven and natural convection flows}
A growing body of work has applied PINNs specifically to natural and turbulent convection. Cai et al.\ \citep{cai2021heat} surveyed PINN applications to a range of heat-transfer problems, including convection-diffusion, and highlighted their ability to solve ill-posed problems -- e.g., inferring temperature or velocity fields from sparse or indirect measurements -- that are difficult for conventional CFD. Lucor, Agrawal, and Sergent \citep{lucor2022} developed PINN surrogates for turbulent Rayleigh--B\'{e}nard convection by combining sparse DNS temperature/velocity data with the governing PDE residual, and introduced simple padding and normalization strategies that substantially improved accuracy near domain boundaries. Fowler, McDevitt, and Roy \citep{fowler2024} solved the two-dimensional differentially heated cavity with a PINN built on a vorticity--streamfunction formulation of the Navier--Stokes equations and reported solutions validated against classical benchmark data over a Rayleigh-number range comparable to the one considered here. These studies collectively demonstrate that, with an appropriate architecture, loss formulation, and (in several cases) auxiliary data, PINNs can reproduce natural-convection solutions to good accuracy. None of them, however, varies the non-dimensionalization of the governing equations as an independent factor while holding the network, training procedure, and data budget fixed, so the effect we document here -- that this single choice can be the difference between a well-converged solution and outright divergence -- has not, to our knowledge, been previously isolated.

\subsection{Classical benchmarks for the differentially heated cavity}
The square, differentially heated cavity has served as a standard validation problem for buoyancy-driven flow solvers since de Vahl Davis \citep{devahldavis1983} published a benchmark-quality finite-difference solution at $\mathrm{Pr}=0.71$ for $\mathrm{Ra}=10^3$--$10^6$. Wan, Patnaik, and Wei \citep{wan2001} later extended this benchmark up to $\mathrm{Ra}=10^8$ using two independent high-accuracy schemes (a discrete-singular-convolution method and a finite-element method), and additionally cautioned that comparing solvers only on scalar summary quantities such as the maximum velocity or average Nusselt number ``could lead to erroneous conclusions,'' since two visibly different solutions can share the same extremal values -- a point we return to in Section~\ref{sec:results}. We use their tabulated values, together with an independently generated DNS solution at the same $(\mathrm{Ra},\mathrm{Pr})$ (Section~\ref{sec:formulation}), as ground truth throughout this paper.

\subsection{Contribution of this work}
Natural convection in a differentially heated cavity is a natural setting in which to isolate the effect of non-dimensionalization on PINN trainability, because the steady Boussinesq equations admit two textbook non-dimensionalizations of the same physics. A thermal-diffusive velocity scale $U=\alpha/L$ -- used in the classical benchmarks above -- gives a buoyancy term in the momentum equation with a coefficient of $\mathrm{Ra}\,\mathrm{Pr}$. A free-fall (buoyancy) velocity scale $U=\sqrt{g\beta\Delta T L}$ instead gives a buoyancy coefficient of exactly~1, at the cost of viscous and thermal-diffusive coefficients that scale as $\sqrt{\mathrm{Pr}/\mathrm{Ra}}$ and $1/\sqrt{\mathrm{Ra}\,\mathrm{Pr}}$. Both are algebraically exact restatements of the same problem, so a numerical method that resolves the equations to convergence should, in principle, be indifferent to the choice. We show that a PINN is not: with everything else held fixed -- network architecture, collocation-point budget, optimizer, and iteration count -- the diffusive scaling produces a PINN that is 157--650\% in error on the average Nusselt number, or diverges outright, over exactly the Rayleigh-number range ($\mathrm{Ra}=10^3$--$10^5$, $\mathrm{Pr}=0.71$) where the free-fall scaling trains cleanly and matches an independent DNS solution to a few percent. We trace this to a gradient-scale imbalance rooted directly in the PDE's buoyancy coefficient -- distinct from, and arising prior to, the inter-loss-term imbalances addressed by the mitigation strategies reviewed in Section~\ref{sec:pathologies} -- and argue that non-dimensionalization should be treated as a first-order design choice for PINNs applied to buoyancy-driven flow.

The remainder of this note is organized as follows. Section~\ref{sec:formulation} states the governing equations solved by both the DNS reference and the PINN, under both non-dimensionalizations. Section~\ref{sec:methods} describes the PINN architecture, the hard-constrained boundary conditions, and the training procedure, held identical across all comparisons. Section~\ref{sec:results} presents the convergence behavior, the quantitative comparison against DNS and the literature benchmark of Wan et al.\ \citep{wan2001}, and the qualitative flow structure. Section~\ref{sec:discussion} discusses the mechanism and its implications, and Section~\ref{sec:conclusion} concludes.


==> results_old.tex <==
In this section, we first discuss the training convergence, followed by accuracy of the PINN results and flow structures. In addition, we show that the two well-known remedies for the gradient imbalance in the loss do not solve the training problems. 

\subsection{Training convergence}
We begin our discussion with the comparison of convergence between diffusive and free-fall PINNs. In Fig.~\ref{fig:convergence}, we show the PDE residual loss during training for both the scalings at increasing $Ra$. While in the free-fall case, the loss decreases smoothly and monotonically, and reaches $1.8\times10^{-5}$, $6.4\times10^{-5}$, and $4.8\times10^{-4}$ at $\mathrm{Ra}=10^3,10^4,10^5$, respectively. Note that a spike at 5000 iteration is due to change in the optimiser from Adam to L-BFGS. Also, with increasing $Ra$, the initial loss increases which indicates the need for higher iteration for higher $Ra$ cases. 

On the other hand, the diffusive loss plateaus 3--8 orders of magnitude higher under Adam at every Ra. At $\mathrm{Ra}=10^5$, the loss rises abruptly and diverges during L-BFGS, see the spike toward $10^{16}$ in Fig.~\ref{fig:convergence}c. Note that the loss term in $Ra=10^3$ and $10^4$ appears to have a final loss of several orders higher than the free-fall loss (12.1, 5079, and \texttt{NaN}).

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/convergence_comparison.png}
\caption{PDE residual loss vs.\ training iteration (Adam, iterations 0--5{,}000, then L-BFGS) for the diffusive and free-fall non-dimensionalizations at (a) $\mathrm{Ra}=10^3$, (b) $\mathrm{Ra}=10^4$, (c) $\mathrm{Ra}=10^5$. The diffusive curve in (c) diverges to \texttt{NaN} during L-BFGS.}
\label{fig:convergence}
\end{figure}

\subsection{Accuracy comparison against DNS}
We further compare the accuracy of DNS results with PINNs. Table~\ref{tab:dns} shows the error in global $\bar{Nu}$, and error in maximum $u$ and $v$. From $Ra=10^3$ to $10^5$, error in $\bar{Nu}$ increases for both the scalings. While the differences in free-fall scaling is in acceptable range up to $Ra=10^4$, diffusive-scaling gives huge error even at smallest $Ra$. Note that we have restricted the maximum number of iterations for all the cases, which is responsible for a $11.5\%$ error in $\bar{Nu}$ at $Ra=10^5$. As a cross-check, the DNS value $\overline{\mathrm{Nu}}=1.101$ at $\mathrm{Ra}=10^3$ agrees within 2.6\% with the value 1.073 reported by Wan et al.\ \citep{wan2001}.

Compared to $\overline{\mathrm{Nu}}$, maximum error in $u$ and $v$ is relatively less but significantly high from the reference cases. It is important to mention that the PDE residual loss trend is similar in diffusive and free-fall scaling at least for the two lower $Ra$ cases but their higher magnitude would need more number of iterations to converge to the reference results. 
% The diffusive PINN is 157.7\% and 648.5\% in error at $\mathrm{Ra}=10^3$ and $10^4$, and gives no usable result at $\mathrm{Ra}=10^5$. 
% , which  the error can be reduced with more number of iterations. the differences are significantly larger in diffusive scaling case. 
% , whereas the free-fall scaling results in the compares  The free-fall PINN is within 1.1\% of DNS in $\overline{\mathrm{Nu}}$ at $\mathrm{Ra}=10^3$ and $10^4$ and within 11.5\% at $\mathrm{Ra}=10^5$. 


\begin{table}[t!]
\centering
\caption{Average Nusselt number and global velocity maxima, PINN vs.\ DNS (both evaluated on the $64\times64$ DNS grid). Percent error is relative to DNS. }
% Velocities are compared on the free-fall scale; diffusive values are divided by $\sqrt{\mathrm{Ra}\,\mathrm{Pr}}$.}
\label{tab:dns}
\begin{tabular}{@{}llrrrr@{}}
\toprule
Scaling & $\mathrm{Ra}$ & $\overline{\mathrm{Nu}}$ (DNS) & $\overline{\mathrm{Nu}}$ err.\ (\%) & $u_{\max}$ err.\ (\%) & $v_{\max}$ err.\ (\%) \\
\midrule
Diffusive & $10^3$ & 1.101 & 157.7 & 1.9 & 20.3 \\
Free-fall & $10^3$ & 1.101 & 0.0 & 0.8 & 1.1 \\
\addlinespace
Diffusive & $10^4$ & 2.218 & 648.5 & 84.1 & 54.2 \\
Free-fall & $10^4$ & 2.218 & 1.1 & 0.3 & 0.3 \\
\addlinespace
Diffusive & $10^5$ & 4.492 & \texttt{NaN} & \texttt{NaN} & \texttt{NaN} \\
Free-fall & $10^5$ & 4.492 & 11.5 & 2.4 & 4.3 \\
\bottomrule
\end{tabular}
\end{table}

Wan et al.\ \citep{wan2001} mentioned that the scalar quantities can give misleading results. Therefore, we also compute the full-field relative $L_2$ error over the entire grid, which is defined as 
\begin{equation}\label{eq:fullfield_relativeerror}
    \mathrm{L}_2 = \frac{\|\phi_{\mathrm{PINN}}-\phi_{\mathrm{DNS}}\|_2} {\|\phi_{\mathrm{DNS}}\|_2}
\end{equation}
As listed in Table~\ref{tab:fielderror}, the error grows with $Ra$ for both the diffusive and free-fall scaling PINNs. However, the error remains below $1.5\%$ up to $Ra=10^4$ and the higher error at $Ra=10^5$ is due to limited iterations. 
% The diffusive scaling reaches 95.8\% error in $\theta$ at $\mathrm{Ra}=10^4$, whereas the free-fall scaling stays below 1.3\% for all fields at $\mathrm{Ra}\le10^4$ and below 21\% at $\mathrm{Ra}=10^5$.

\begin{table}[t!]
\centering
\caption{Full-field relative $L_2$ error (Eq. \ref{eq:fullfield_relativeerror}) against DNS over the entire $64\times64$ grid.}
\label{tab:fielderror}
\begin{tabular}{@{}llrrr@{}}
\toprule
Scaling & $\mathrm{Ra}$ & $u$ (\%) & $v$ (\%) & $\theta$ (\%) \\
\midrule
Diffusive & $10^3$ & 22.3 & 41.5 & 54.1 \\
Free-fall & $10^3$ & 1.0 & 1.3 & 0.1 \\
\addlinespace
Diffusive & $10^4$ & 88.7 & 90.7 & 95.8 \\
Free-fall & $10^4$ & 1.0 & 1.2 & 0.9 \\
\addlinespace
Diffusive & $10^5$ & \texttt{NaN} & \texttt{NaN} & \texttt{NaN} \\
Free-fall & $10^5$ & 20.9 & 14.2 & 9.7 \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/freefall_ra1e4_fields.png}
\caption{Free-fall PINN solution at $\mathrm{Ra}=10^4$: (a) temperature, (b) streamfunction, (c) velocity streamlines colored by speed, (d) pressure relative to its mean. Velocity, streamfunction, and pressure are on the free-fall scale.}
\label{fig:fields-freefall}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/diffusive_ra1e4_fields.png}
\caption{Diffusive-scaling PINN solution at $\mathrm{Ra}=10^4$ with the same architecture and training budget as Fig.~\ref{fig:fields-freefall}: (a) temperature, (b) streamfunction, (c) velocity streamlines colored by speed, (d) pressure relative to its mean, all converted to the free-fall scale. The temperature has collapsed to a thin near-wall layer instead of the smooth field of Fig.~\ref{fig:fields-freefall}(a).}
\label{fig:fields-diffusive}
\end{figure}
\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/freefall_ra1e4_dns_compare.png}
\caption{Free-fall PINN vs.\ DNS at $\mathrm{Ra}=10^4$: (a) $u$, (b) $v$, (c) $\theta$. Columns show DNS, PINN, and the absolute pointwise error $|\mathrm{PINN}-\mathrm{DNS}|$. DNS and PINN share one color scale per row.}
\label{fig:dns-freefall}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/diffusive_ra1e4_dns_compare.png}
\caption{Diffusive-scaling PINN vs.\ DNS at $\mathrm{Ra}=10^4$, same layout as Fig.~\ref{fig:dns-freefall}. The PINN panels share the DNS color scale, so the nearly uniform panels reflect genuinely small-amplitude, structurally wrong fields and not a plotting artifact.}
\label{fig:dns-diffusive}
\end{figure}

\subsection{Flow structure comparison}
Differentially heated cavity (DHC) has a well-known recirculating cell at the center of the cavity and a gentle S-shaped temperature field at small $Ra$. Here, we compare the flow structures among the diffusive and free-fall scaling at $Ra=10^4$. 

Figure~\ref{fig:fields-freefall} shows the free-fall PINN solution at $\mathrm{Ra}=10^4$: a temperature field with the gentle S-shaped stratification, a single smooth S-shaped recirculating cell shown by streamfunction and velocity field. On the other hand, as shown in Fig.~\ref{fig:fields-diffusive}, the diffusive PINN significantly deviates from the coherent flow features of DHC. 
Particularly, the temperature collapses to a thin near-wall layer with the bulk at a nearly constant temperature $\theta\approx0$. The recirculating core deviates from the center as shown in the streamfunction and flow field. 
Note that the pressure field is quite smooth in free-fall scaling, whereas, it exhibits dual peaks close to the left wall in the diffusive case. 

Next, we show a direct comparison of the PINN results with the DNS at $\mathrm{Ra}=10^4$ in Figs.~\ref{fig:dns-freefall} and \ref{fig:dns-diffusive}. Qualitatively, it is difficult to distinguish between the free-fall PINN from DNS for all three fields. In fact, the pointwise error is more than two orders of magnitude smaller than the field values. On the other hand, the diffusive PINN fails to reproduce the coherent flow structures. Although the $u$ and $v$ field shows very weak features close to the walls, their magnitude is six times smaller than the values in DNS. Temperature field shows the worst features without any S-shaped stratified structure, and the error in $\theta$ exceeds $0.5$ over most of the domain. 
% At $\mathrm{Ra}=10^5$, the weights of the diffusive PINN are \texttt{NaN} throughout and no field can be plotted, a direct consequence of the divergence in Fig.~\ref{fig:convergence}(c).

Therefore, the diffusive PINNs are difficult to train not just in accuracy but also reproducing the well-known flow features. However, the free-fall scaling is suitable for the PINN architecture. 


\subsection{Mechanism: amplification of gradient imbalance}
\label{sec:discussion}

The previous studies used a scaling that gives $B\approx 1$ \cite{cai2021heat,volk_pinn_2025}. However, a proper reasoning is required for the choice because of different coefficients associated with diffusion and buoyancy, which enters the loss terms. To resolve this issue, we decompose the loss function of y-momentum equation to check the gradient imbalance causing terms. 
% losses in terms of discuss the mechanism responsible for training issues in the PINNs for buoyancy driven flow. Due to different scaling, we obtain different coefficients of the terms in loss of the PDE, see Table \ref{tab:scalinglaw}, which creates a gradient imbalance during optimization. 
% The trivial field $\theta\equiv0$, $u=v\equiv0$, $p\equiv\mathrm{const}$ is a near-zero-residual point of the interior PDE loss in both scalings. 
% In the present hard-constrained network, $\theta$ cannot be zero everywhere, but it starts close to, and remains for a long time near, the pure-conduction profile $\theta\approx1-x$. At initialization the raw outputs $\psi_{\mathrm{raw}}$ and $\theta_{\mathrm{raw}}$ are small (Xavier-normal weights, zero bias), so $u\approx v\approx0$ and $\theta\approx1-x$ is set almost entirely by the affine term of the hard constraint. What differs between the two scalings is the cost of leaving this near-conductive state for the true convecting solution.
The $y$-momentum residual can be written as $\mathrm{mom}_v = R - B\,\theta$, where $R$ collects the advection, pressure, and viscous terms, while $B=\mathrm{Ra}\,\mathrm{Pr}$ in the diffusive scaling and $B=1$ in the free-fall scaling (Eqs.~\ref{eq:diff-momy}, \ref{eq:ff-momy}). Near initialization, $u,v\approx0$ and $\theta = O(1)$, so $R$ is small and $\mathrm{mom}_v \approx -B\theta$. With $\mathcal{L}_v = \mathrm{mom}_v^2$, the gradient with respect to a network weight $w$ is
\begin{align}
\frac{\partial \mathcal{L}_v}{\partial w} &= 2\,\mathrm{mom}_v\,\frac{\partial\, \mathrm{mom}_v}{\partial w} \nonumber \\
&\approx 2(-B\theta)(-B)\frac{\partial \theta}{\partial w} = 2B^2\,\theta\,\frac{\partial \theta}{\partial w}.
\label{eq:gradscaling}
\end{align}

Note that $B$ enters twice, once through the magnitude of the residual and once through its derivative. The gradient directs $\theta$ toward the conduction state, which scales as $B^2$, relative to the fixed-weight boundary-condition, which are the only terms pulling $\theta$ toward its correct values. Since $B=\mathrm{Ra}\,\mathrm{Pr}$ in the diffusive scaling, $B^2$ grows by two orders of magnitude for every decade of Ra (Table~\ref{tab:scalinglaw}). This argument closely follows the severity observed in Table~\ref{tab:dns}, i.e., a finite but large error at $\mathrm{Ra}=10^3,10^4$ and $NaN$ at $10^5$. On the other hand, in the free-fall scaling $B=1$ at every Ra. Consequently, the amplification of the gradient imbalance is absent. Note that the viscous and diffusive coefficients decrease (Table~\ref{tab:coefficients}) with $Ra$, which corresponds to thinner boundary layers. Such scenarios can be addressed with more resolution on the collocation points, and does not create an optimization pathology.

\begin{table}[t!]
\centering
\caption{Gradient-amplification factor $B^2$ predicted by Eq.~\eqref{eq:gradscaling} for the diffusive scaling ($B=\mathrm{Ra}\,\mathrm{Pr}$), together with the PINN error from Table~\ref{tab:dns}. $B^2$ grows by two orders of magnitude per decade of Ra, following the observed progression from large but finite error to divergence.}
\label{tab:scalinglaw}
\begin{tabular}{@{}lrrl@{}}
\toprule
$\mathrm{Ra}$ & $B=\mathrm{Ra}\,\mathrm{Pr}$ & $B^2$ & Diffusive $\overline{\mathrm{Nu}}$ error \\
\midrule
$10^3$ & 710 & $5.0\times10^5$ & 157--169\% \\
$10^4$ & 7{,}100 & $5.0\times10^7$ & 619--695\% \\
$10^5$ & 71{,}000 & $5.0\times10^9$ & \texttt{NaN} (diverged) \\
\bottomrule
\end{tabular}
\end{table}

We verify the proposed mechanism at a fixed $Ra=10^4$ by decomposing and directly measuring the loss terms. The network is re-initialized with the same seed and architecture for both scalings. As shown in Fig.~\ref{fig:gradnorm}, the $L_2$ norm of the gradient with respect to network parameters is computed for each of the five raw, unweighted loss terms (two momentum residuals, energy residual, no-slip, adiabatic) at logged intervals over 500 Adam iterations. Interestingly, in the diffusive scaling, the $y$-momentum (buoyancy) gradient starts at $8.35\times10^8$ times the no-slip gradient and stays 5--7 orders of magnitude above every boundary term for all 500 iterations, see Fig.~\ref{fig:gradnorm}a. Clearly, the gradient imbalance persists and does not resolve with training. 
It is of the same order as the prediction $B^2=5.0\times10^7$.
% the remaining factor of about 17 reflects architecture- and initialization-specific constants not captured by the leading-order argument. 
On the other hand, as shown in Fig.~\ref{fig:gradnorm}b), in the free-fall scaling, the same ratio at initialization is of order ($10$), consistent with $B^2=1$. By iteration 100, the $x$- and $y$-momentum gradients collapses and agree within a few percent, whereas the remaining three terms drops to at least two orders of magnitude. 

Note that these are unweighted gradients, and no fixed loss weight in the diffusive scaling can close a gap of $10^6$--$10^8$, wherein the boundary terms are already weighted 20 times. Therefore, the gradient imbalance needs to be removed at the level of the PDE coefficients, which demands a $B\approx O(1)$. This conditions is satisfied not only by the free-fall scaling but a few others, which are used by \cite{cai2021heat,volk_pinn_2025}.

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/grad_diag_ra1e4.png}
\caption{$L_2$ norm of the gradient (with respect to all network parameters) of each of the five raw, unweighted loss terms at $\mathrm{Ra}=10^4$ over 500 Adam iterations from a common seeded initialization: (a) diffusive scaling, (b) free-fall scaling. Note the different vertical scales: the diffusive $y$-momentum term never drops below $10^5$, whereas every free-fall term stays within $10^{-4}$--$10^0$.}
\label{fig:gradnorm}
\end{figure}

We acknowledge that this is a specific instance of the gradient imbalance between competing loss terms studied by Wang et al.\ \citep{wang2021}. Here, however, it arises purely from the non-dimensionalization, before any inter-term weighting is applied. Consequently, the gradient imbalance associated with a coefficient sits inside the PDE residual itself. To test our argument, we have tested both the remedies: the data loss and self-adaptive weighting. We have provided 20 sparse DNS points for supervision with a weight of 20. It is found that the supervision changes the flow results by at most a few percentage points on an error that was 80--95\%, see Table~\ref{tab:data}. Therefore, the gradient-norm-based adaptive weighting either left the field unchanged or suppressed the buoyancy term Table~\ref{tab:adaptive}. 
Reweighting redistributes the gradient among loss terms but does not remove the $B^2$ factor inside the residual. Likewise, the hard boundary conditions of Sec.~\ref{sec:methods} fixed the more severe failure of convergence to the trivial state under soft conditions, but Table~\ref{tab:dns} shows that they are insufficient once $\mathrm{Ra}\,\mathrm{Pr}$ is large enough, since the imbalance returns as a slow, biased convergence of the interior residual.

For buoyancy-driven and other multi-physics problems where the non-dimensionalization can be chosen freely, the practical implication is that the choice should be treated as a hyperparameter on the same footing as the architecture and the loss weights. A free-fall-type scaling, which keeps every coefficient $O(1)$ or smaller over the parameter range of interest, is a zero-cost mitigation that requires no change in the network, optimizer, or loss weights.

% \paragraph{Limitations} The steady study uses a single architecture, a single random seed per configuration, and a fixed collocation-point budget. A broader sweep over seeds, network sizes, and adaptive point refinement, particularly for the thinning boundary layers at higher Ra, would strengthen the generality of the trend. We restrict the comparison to $\mathrm{Ra}\le10^5$; at higher Ra the error of the free-fall scaling is expected to grow as a resolution effect, which is a separate question from the trainability failure of the diffusive scaling. The data study is limited to one Rayleigh number, one data location and count (20 points along one vertical line), and one data weight, and we did not test whether a much denser data set could overcome the imbalance. Our claim is only that a substantial, realistically weighted sparse-data signal did not. The adaptive-weighting study carries the three caveats listed in Sec.~\ref{sec:adaptive-setup}, and a sweep over $\alpha$, the update interval, and the reference statistic, together with an exact reproduction of the original per-layer formulation, is needed for a sharper statement on that method. The unsteady study is limited to one Rayleigh number, free-fall scaling only (the diffusive scaling was not run), two seeds, one time horizon, and one initial condition; the missing Nusselt-number overshoot may depend on the training budget, the number of time bins, and the sampling near $t=0$, none of which were varied. 

\section{Handling the situation}
\subsection{Effect of sparse data assimilation}
\label{sec:data-results}
Next, we evaluate the two well-known strategies to handle the imbalance. Table~\ref{tab:data} reports the full-field error and the hot-wall $\overline{\mathrm{Nu}}$ for the six configurations of Sec.~\ref{sec:data-setup}. $\overline{\mathrm{Nu}}$ is obtained by integrating $\mathrm{Nu}_{\mathrm{local}}(y)=-\partial\theta/\partial x|_{x=0}$, evaluated exactly by automatic differentiation. Sparse data change almost nothing for the diffusive scaling. Velocity-only supervision reduces the error in $u$ from 88.7\% to 82.0\% and in $v$ from 90.7\% to 83.2\%, but the error in $\theta$ remains 95.0\% and $\overline{\mathrm{Nu}}$ is still off by more than 600\%. Adding temperature supervision ($\tau=1$) does not help either; the error in $\theta$ is marginally higher (95.3\%) even though $\theta$ is now supervised directly at 20 points. In contrast, the free-fall scaling continues to improve with supervision: the error in $\theta$ decreases from 0.92\% (no data) to 0.41\% ($\tau=0$) and 0.26\% ($\tau=1$). Thus, data improve a solution that physics has already made accurate, but cannot repair one that the optimization has failed to find.

\begin{table}[htbp]
\centering
\caption{Full-field relative $L_2$ error against DNS and hot-wall average Nusselt number for different data conditions at $\mathrm{Ra}=10^4$: no data (main study), sparse velocity data ($\tau=0$, 20 points at $x\approx0.5$), and sparse velocity and temperature data ($\tau=1$, same points).}
\label{tab:data}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Scaling & Data condition & $u$ (\%) & $v$ (\%) & $\theta$ (\%) & $\overline{\mathrm{Nu}}$ & $\overline{\mathrm{Nu}}$ err.\ (\%) \\
\midrule
Diffusive & No data & 88.7 & 90.7 & 95.8 & 17.13 & 672 \\
Diffusive & $\tau=0$ (u,v) & 82.0 & 83.2 & 95.0 & 15.95 & 619 \\
Diffusive & $\tau=1$ (u,v,$\theta$) & 82.5 & 84.3 & 95.3 & 15.85 & 614 \\
\addlinespace
Free-fall & No data & 0.98 & 1.24 & 0.92 & 2.272 & 2.40 \\
Free-fall & $\tau=0$ (u,v) & 0.61 & 1.16 & 0.41 & 2.252 & 1.53 \\
Free-fall & $\tau=1$ (u,v,$\theta$) & 0.57 & 1.06 & 0.26 & 2.250 & 1.41 \\
\bottomrule
\end{tabular}
\end{table}

The data are not simply inert for the diffusive scaling; they distort the flow topology. Figure~\ref{fig:data-fields} shows that, with velocity data, the temperature remains collapsed as in the no-data case (compare Fig.~\ref{fig:fields-diffusive}a), but the streamfunction now contains a spurious two-vortex structure, with a small cell near $x\approx0.2$ and a larger one near $x\approx0.55$. This is unphysical at $\mathrm{Ra}=10^4$, since Wan et al.\ \citep{wan2001} report that the core splits into two counter-rotating eddies only around $\mathrm{Ra}=10^5$. The data perturb the streamfunction locally near the data line, while the rest of the domain remains governed by the same failed optimization. The resulting solution is arguably more misleading than the no-data case, because the additional flow structure looks plausible but is not more accurate.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/diffusive_ra1e4_data_fields.png}
\caption{Diffusive-scaling PINN with sparse velocity data ($\tau=0$) at $\mathrm{Ra}=10^4$: (a) temperature, (b) streamfunction, (c) velocity streamlines colored by speed, (d) pressure relative to its mean, all on the free-fall scale. In contrast to the single off-center vortex of the no-data case (Fig.~\ref{fig:fields-diffusive}b,c), the data introduce a spurious second vortex core.}
\label{fig:data-fields}
\end{figure}

The same conclusion follows from the local Nusselt number $\mathrm{Nu}_{\mathrm{local}}(y) = -\partial\theta/\partial x$ at the hot ($x=0$) and cold ($x=1$) walls (Fig.~\ref{fig:nusselt-data}). At the hot wall, all three diffusive curves are 5--15 times larger than DNS and share the same wrong shape, flat in the middle of the wall and spiking at both ends, instead of the smooth monotonic decay of DNS. The three curves are nearly indistinguishable regardless of the data supplied. At the cold wall, the diffusive curves are close to zero, whereas DNS decays smoothly from about 3.5 to 0.6. The free-fall curves are within a few percent of DNS at both walls for all three data conditions. Note that the hot- and cold-wall $\overline{\mathrm{Nu}}$ of DNS agree within 0.005\% (2.2184 and 2.2183), as required by the steady heat balance. The free-fall PINN preserves this balance reasonably well (2.21--2.27 at both walls), but the diffusive PINN does not (17 at the hot wall and nearly 0 at the cold wall). The diffusive solution is thus not only inaccurate but also violates energy conservation across the domain, irrespective of the sparse data supplied.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/nusselt_comparison_data.png}
\caption{Local Nusselt number $\mathrm{Nu}_{\mathrm{local}}(y)=-\partial\theta/\partial x$ at the hot wall ($x=0$, top row) and cold wall ($x=1$, bottom row) at $\mathrm{Ra}=10^4$, comparing DNS (symbols) with the three data conditions for each scaling: no data (dotted), $u,v$ data (dashed), and $u,v,\theta$ data (solid).}
\label{fig:nusselt-data}
\end{figure}

\subsection{Effect of adaptive loss weighting}
\label{sec:adaptive-results}
Table~\ref{tab:adaptive} reports the five Adam-only runs of Sec.~\ref{sec:adaptive-setup}. Neither scheme rescues the diffusive scaling. The coarse scheme leaves the field error indistinguishable from the fixed-weight baseline (both $\approx$100\% in $u$ and $v$) and makes $\overline{\mathrm{Nu}}$ worse (40.7 vs.\ 29.3, against the DNS value of 2.218). The final weights show why: $\lambda_{\mathrm{vel}}$ and $\lambda_\theta$ are driven to $1.1\times10^{10}$ and $7.4\times10^{11}$, which satisfies the boundary conditions to a precision that was never the binding constraint, while the $y$-momentum term, which the scheme cannot reweight, remains as dominant as before. A scheme that treats the PDE residual as one group cannot correct an imbalance that lives inside that group.

\begin{table}[htbp]
\centering
\caption{Adaptive loss weighting at $\mathrm{Ra}=10^4$: full-field relative $L_2$ error against DNS, hot-wall $\overline{\mathrm{Nu}}$ (DNS value 2.218), and the final adapted weight of the $y$-momentum term. All runs are Adam-only with 5{,}000 iterations, so the errors are not comparable to Tables~\ref{tab:dns}--\ref{tab:data}; the fixed-weight rows are the matched-budget controls. $\overline{\mathrm{Nu}}=1$ is the exact pure-conduction (no-flow) limit.}
\label{tab:adaptive}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Scaling & Weighting & $u$ (\%) & $v$ (\%) & $\theta$ (\%) & $\overline{\mathrm{Nu}}$ & final $\lambda_{\mathrm{mom}_v}$ \\
\midrule
Diffusive & Fixed (control) & 99.7 & 104.5 & 100.1 & 29.26 & 1 \\
Diffusive & Adaptive, coarse & 100.0 & 100.0 & 97.5 & 40.69 & 1 \\
Diffusive & Adaptive, fine & 100.0 & 100.0 & 89.9 & 9.97 & $7.8\times10^{-6}$ \\
\addlinespace
Free-fall & Fixed (control) & 11.0 & 15.1 & 16.7 & 2.807 & 1 \\
Free-fall & Adaptive, fine & 99.5 & 99.6 & 36.9 & 1.016 & $2.2\times10^{-3}$ \\
\bottomrule
\end{tabular}
\end{table}

The fine scheme can rebalance within the PDE group, but it does not help either, and its failure is more instructive. Gradient balance is achieved by suppressing the $y$-momentum equation: $\lambda_{\mathrm{mom}_v}$ falls from 1 to $7.8\times10^{-6}$ while the raw residual remains $O(10^6)$. The balance is obtained by abandoning the term and not by solving it.

The clearest evidence that this is a genuine pathology and not a feature of the failed diffusive case is that the same scheme destroys the free-fall solution, which trains well without it. Fine-grained annealing raises the velocity error of the free-fall run from 11--15\% (fixed-weight control) to $\approx$100\% and drives $\overline{\mathrm{Nu}}$ to 1.016. This value is diagnostic: $\overline{\mathrm{Nu}}=1$ is the pure-conduction limit, obtained when the fluid is motionless and $\theta=1-x$. The run has therefore converged to the no-convection solution. The final weight $\lambda_{\mathrm{mom}_v}=2.2\times10^{-3}$ explains this. The $y$-momentum equation is the only place where buoyancy enters, and hence the only coupling between temperature and flow. A heuristic that identifies it as the largest-gradient term and suppresses it removes the sole driver of convection, after which the optimizer can satisfy all remaining terms while solving a problem that no longer contains the phenomenon of interest.

Two conclusions follow. First, adaptive loss weighting is not an alternative to choosing a suitable non-dimensionalization for this problem, at either granularity and at matched budget. Second, gradient-magnitude balancing is not a safe default when one loss term carries the physics that couples an otherwise inert system. The caveats of Sec.~\ref{sec:adaptive-setup} bound the second conclusion; in particular, the down-weighting pathology arises in our generalization, since the published scheme holds the PDE-residual weight fixed.


\section{Time evolution of the flow field}
\label{sec:unsteady-results}
Figure~\ref{fig:unsteady-nu}(a) compares the average Nusselt number at the hot wall, $\overline{\mathrm{Nu}}(t)$, with the reference. In the reference, $\overline{\mathrm{Nu}}$ starts at 1 (pure conduction), rises to a maximum of 2.408 at $t=5.4$, falls to a minimum of 2.222 at $t=9.9$, and settles at 2.245. The PINN reproduces the start-up and the final state: $\overline{\mathrm{Nu}}(20)$ is 2.232 and 2.261 for the two seeds, which is $-0.6\%$ and $+0.7\%$ from the steady reference value. However, it does not reproduce the overshoot. Both seeds rise smoothly to about 2.30 at $t\approx10$--12 and then decay slowly, so the oscillation of amplitude about 0.19 in the reference is missing. The PINN also leads the reference in the rise, and the maximum error in $\overline{\mathrm{Nu}}$ is 0.33 (seed 0) and 0.30 (seed 1) near $t\approx2$, where the reference value is only about 1.2--1.3, so the relative error is 23--27\%. In addition, both seeds dip below $\overline{\mathrm{Nu}}=1$ (to 0.92 and 0.90 at $t\approx0.3$), which the reference does not show. This smoothing of a sharp temporal feature is consistent with the known tendency of PINNs to favor smooth solutions, but we have not tested a remedy.

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/unsteady_nu_errors.png}
\caption{Unsteady flow from rest at $\mathrm{Ra}=10^4$ (free-fall scaling): (a) average Nusselt number at the hot wall, reference and two PINN seeds; (b) relative $L_2$ error of $\theta$, $u$, and $v$ against the reference at the times of the stored reference snapshots (filled symbols: seed 0; open symbols: seed 1).}
\label{fig:unsteady-nu}
\end{figure}

The field errors in Fig.~\ref{fig:unsteady-nu}(b) and Table~\ref{tab:unsteady} show the same pattern. The relative error in $\theta$ is 2--8\% during the transient ($t\le5$) and falls to 1--2\% at $t=20$. The velocity errors are larger: they are 13--26\% at $t=0.5$ and about 20\% at $t=2$--3, when the buoyancy-driven circulation accelerates, and they fall to 2--4\% for $t\ge12$. Figure~\ref{fig:unsteady-fields} shows that the temperature fronts and the streamlines nevertheless have the correct structure at all times, with the vortex core located and shaped correctly at $t=20$. The remaining differences are small displacements of the thermal boundary layers at early times and a slightly weaker circulation at $t=3$.

\begin{table}[t!]
\centering
\caption{Unsteady flow from rest at $\mathrm{Ra}=10^4$: error of the PINN (two seeds) against the finite-difference reference. $\overline{\mathrm{Nu}}(20)$ is compared with the reference value 2.245; the mean and maximum of $|\Delta\overline{\mathrm{Nu}}|$ are taken over $0\le t\le20$; the last six columns are relative $L_2$ errors (\%) over the whole grid.}
\label{tab:unsteady}
\small
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
 & & \multicolumn{2}{c}{$|\Delta\overline{\mathrm{Nu}}|$} & \multicolumn{3}{c}{$t=3$} & \multicolumn{3}{c}{$t=20$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Seed & $\overline{\mathrm{Nu}}(20)$ & mean & max & $u$ & $v$ & $\theta$ & $u$ & $v$ & $\theta$ \\
\midrule
0 & 2.232 & 0.090 & 0.334 & 21.8 & 22.0 & 6.5 & 3.6 & 3.2 & 1.3 \\
1 & 2.261 & 0.079 & 0.302 & 19.1 & 19.5 & 5.1 & 2.3 & 3.2 & 1.9 \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{figures/unsteady_fields.png}
\caption{Temperature (filled contours) and streamfunction (dashed lines) at $t=1,3,5,20$ for the reference (top row) and the PINN with seed 0 (bottom row), $\mathrm{Ra}=10^4$, free-fall scaling.}
\label{fig:unsteady-fields}
\end{figure}

Thus, with the free-fall scaling a PINN started from rest finds the correct steady heat transfer and flow structure without any data, but its time-accurate behavior is only moderately accurate: the overshoot of the Nusselt number is not captured and the velocity errors in the transient are an order of magnitude larger than at steady state. The comparison with the steady cases of Table~\ref{tab:dns} (errors of about 1\% at the same Ra) shows that the time-dependent problem is considerably harder for the same network size and training budget.

